Sparse Backpropagation for MoE Training

One defining characteristic of Mixture-of-Expert (MoE) models is their capacity for conducting sparse computation via expert routing, leading to remarkable scalability. However, backpropagation, the cornerstone of deep learning, requires dense computation, thereby posting challenges in MoE gradient computations. Here, we introduce SparseMixer, a scalable gradient estimator that bridges the gap between backpropagation and sparse expert routing. Unlike typical MoE training which strategically neglects certain gradient terms for the sake of sparse computation and scalability, SparseMixer provides scalable gradient approximations for these terms, enabling reliable gradient estimation in MoE training. Grounded in a numerical ODE framework, SparseMixer harnesses the mid-point method, a second-order ODE solver, to deliver precise gradient approximations with negligible computational overhead. Applying SparseMixer to Switch Transformer on both pre-training and machine translation tasks, SparseMixer showcases considerable performance gain, accelerating training convergence up to 2 times.

==> input/old_3_method.tex <==
% \section{ST Revisited and Scalable Gradient Approximation}
\section{From Discrete to Sparse: \ours}
\label{sec:sparse}
% Here, we first revisit the derivations for positioning $\appnabla_{\mbox{\scriptsize ST}}$ as a first-order approximation. 
Although ST estimators bridged discrete variables and backpropagation, they require the network to be densely activated. 
Here, we first discuss the intrinsic limitation of ST estimators.
Then, we go beyond discrete and bridge sparse expert routing and backpropagation. 
% estimate gradients without sacrificing the scalability. 

% \subsection{ST Revisited}
% \subsection{Dense Computation of Existing ST Estimators}
\subsection{Why Existing ST Estimators are not Scalable?}
% In \citet{Liu2023BridgingDA}, 
% we positioned $E[\appnabla_{\mbox{\scriptsize ST}}]$ as a first-order approximation of $\nabla_0$ by leveraging~\footnote{Note that $\sum_i E[g] \frac{\partial\,\vpi_{\mI_i}}{\partial\,W_r} = E[g] \frac{\partial\,\sum_{\mI_i} \vpi_{\mI_i}}{\partial\,W_r}=E[g] \frac{\partial\,\bm{1}}{\partial\,W_r}=0$}:
\citet{Liu2023BridgingDA} formally establishes that $E[\appnabla_{\mbox{\scriptsize ST}}]$ 
% is positioned 
is a first-order approximation of $\nabla_0$ by using\footnote{Commonly referred to as baseline subtraction. Note $\sum_i E[g] \frac{\partial\,\vpi_{\mI_i}}{\partial\,W_r} = E[g] \frac{\partial\,\sum_{\mI_i} \vpi_{\mI_i}}{\partial\,W_r}=E[g] \frac{\partial\,\bm{1}}{\partial\,W_r}=0$.}:
\begin{eqnarray}
    \nabla_0 =  \sum_{\mI_i} (g(\pi_{\mI_i} f_{\mI_i}) - E[g]) \frac{\partial\,\vpi_{\mI_i}}{\partial\,W_r} = \sum_{\mI_i} \sum_{\mI_j}  \vpi_{\mI_j} (g(\vpi_{\mI_i}f_{\mI_i}) - g(\vpi_{\mI_j}f_{\mI_j})) \frac{\partial\,\vpi_{\mI_i}}{\partial\,W_r}.
    \label{eqn:st_baseline}
\end{eqnarray}
Specifically, approximating $g(\vpi_{\mI_i}f_{\mI_i}) - g(\vpi_{\mI_j}f_{\mI_j})$ as $g'(\vpi_{\mI_j}f_{\mI_j}) \cdot (\vpi_{\mI_i}f_{\mI_i} - \vpi_{\mI_j}f_{\mI_j})$, the resulting gradient approximation will have the same form as $E[\appnabla_{\mbox{\scriptsize ST}}]$~\citep{Liu2023BridgingDA}.  
In numerical analyses, this approximation is known as the forward Euler method (briefly introduced in Appendix~\ref{appendix:ode}), which has first-order accuracy. 
% We also 
\citet{Liu2023BridgingDA} also 
explored higher-order ODE solvers to better approximate $g(\vpi_{\mI_i}f_{\mI_i}) - g(\vpi_{\mI_j}f_{\mI_j})$. 
However, all these approximations involve both activated experts (i.e., $f_{\mI_j}$) and unactivated experts (i.e., $f_{\mI_j}$), thus contradicting scalability. 
In order words, although those ST estimators bridge discrete and backpropagation, their computations are dense instead of sparse. 

\subsection{Expert Routing Gradient Approximation: Backpropagation Made Sparse}
To bridge the gap between sparse MoE routing and back-propagation, we need to approximate $\nabla_0$ without requiring outputs from all experts. 
In our study, we present a novel framework to move beyond ST and bridge backpropagation and sparse expert routing. 

Here, we start by introducing the most simple gradient estimator, i.e., $\appnabla_{\mbox{\scriptsize \ours-1st}}$, where
\begin{eqnarray*}
\appnabla_{\mbox{\scriptsize \ours-1st}} := \frac{\partial g(\pi_\mD f_\mD(\vx))}{\partial\,W_r}.
\end{eqnarray*}
Similar to $E[\appnabla_{\mbox{\scriptsize ST}}]$, $E[\appnabla_{\mbox{\scriptsize \ours-1st}}]$ is a first-order approximation of $\nabla_0$.
To demonstrate this, we take an alternative approach to rewrite $\nabla_0$:
\begin{eqnarray}
    \nabla_0 =  \sum_{\mI_i} (g(\pi_{\mI_i} f_{\mI_i}) - g(\mZero)) \frac{\partial\,\vpi_{\mI_i}}{\partial\,W_r}.
    \label{eqn:fastmax_baseline}
\end{eqnarray}

Adopting the Euler method, we estimate $g(\vpi_{\mI_i} f_{\mI_i}) - g(\mZero)$ as $g'(\vpi_{\mI_i} f_{\mI_i}) \cdot \vpi_{\mI_i} f_{\mI_i}$.
Comparing to the first-order approximation of Equation~\ref{eqn:st_baseline}, this first-order approximation only requires the output of one expert. 
Then, it is easy to note:
\begin{eqnarray*}
\nabla_0 \overset{\mathrm{forward\,Euler}}{\approx} \sum_{\mI_i} g'(\vpi_{\mI_i} f_{\mI_i}) \cdot \vpi_{\mI_i} f_{\mI_i} \cdot \frac{\partial\,\vpi_{\mI_i}}{\partial\,W_r} = E_{\mD \sim \vpi}[\frac{\partial g(\pi_\mD f_\mD(\vx))}{\partial\,W_r}] = E[\appnabla_{\mbox{\scriptsize \ours-1st}}].
\end{eqnarray*}
Note that, same with $\appnabla_{\mbox{\scriptsize ST}}$, $\appnabla_{\mbox{\scriptsize \ours-1st}}$ adopts the forward Euler method and achieves first-order accuracy. 
Meanwhile, $\appnabla_{\mbox{\scriptsize \ours-1st}}$ only requires the output of one expert thus not sacrificing scalability, while $\appnabla_{\mbox{\scriptsize ST}}$, as in Equation~\ref{eqn:st}, requires the output of all experts. 

\subsection{Achieving Second-Order Accuracy with the Mid-point Method}

The literature on numerical methods for differential equations shows that it is possible to achieve higher-order accuracy \emph{without computing higher-order derivatives}.
To furnish accurate gradient approximations, we employ a second-order ODE method, the mid-point method (briefly introduced in Appendix~\ref{appendix:ode}).
Specifically, $\appnabla_{\mbox{\scriptsize \oursrd}}$ is a second-order approximation of $\nabla$, where
\begin{eqnarray*}
\appnabla_{\mbox{\scriptsize \oursrd}} := 2\cdot \frac{\partial g(\frac{\pi_\mD f_\mD(\vx)}{2})}{\partial\,W_r}.
\end{eqnarray*}

To demonstrate the connection between $\appnabla_{\mbox{\scriptsize \oursrd}}$ and the mid-point method, we employ the mid-point method to approximate $g(\pi_{\mI_i} f_{\mI_i}) - g(\mZero)$ as $g'(\frac{\pi_{\mI_i} f_{\mI_i}}{2}) \cdot \pi_{\mI_i} f_{\mI_i}$, which also requires only the output of one expert. 
Similarly, it is easy to note:
\begin{eqnarray*}
\nabla_0 \overset{\mathrm{mid-point}}{\approx} \sum_{\mI_i} g'(\frac{\pi_{\mI_i} f_{\mI_i}}{2}) \cdot \vpi_{\mI_i} f_{\mI_i} \cdot \frac{\partial\,\vpi_{\mI_i}}{\partial\,W_r} = E_{\mD \sim \vpi}[2\cdot \frac{\partial g(\frac{\pi_\mD f_\mD(\vx)}{2})}{\partial\,W_r}] = E[\appnabla_{\mbox{\scriptsize \oursrd}}].
\end{eqnarray*}
% Accordingly, $E[\appnabla_{\mbox{\scriptsize \oursrd}}]$ is a second-order approximation of $\nabla$, where
% \begin{eqnarray*}
% \appnabla_{\mbox{\scriptsize \oursrd}} := 2\cdot \frac{\partial g(\frac{\pi_\mD f_\mD(\vx)}{2})}{\partial\,W_r}.
% \end{eqnarray*}
Notably, it is feasible to employ more advanced ODE solvers like RKF4 and approximate $\nabla_0$ with even higher-order accuracy~\citep{fehlberg1969classical}.
In our experiments, we observe that the mid-point method is accurate enough and decide to stick to the mid-point method for simplicity.
% \input{input/pseudo}

\subsection{Balancing Router Training and Expert Training}
Comparing to $\appnabla_{\mbox{\scriptsize \ours-1st}}$, $\appnabla_{\mbox{\scriptsize \oursrd}}$ provides better gradient estimation for router training.
However, $\appnabla_{\mbox{\scriptsize \oursrd}}$ causes additional difficulties for expert training.
Specifically, $\appnabla_{\mbox{\scriptsize \oursrd}}$ requires to change the MoE output from $\vy \gets \pi_\mD f_\mD(\vx)$ to $\vy \gets \frac{\pi_\mD f_\mD(\vx)}{2}$, leading to a gap between the training ($\vy \gets \frac{\pi_\mD f_\mD(\vx)}{2}$) and the inference ($\vy \gets \pi_\mD f_\mD(\vx)$). 
As discussed in Section~\ref{subsec:ablation}, such gap 
% $\appnabla_{\mbox{\scriptsize \oursrd}}$ 
creates significant obstacles for MoE training. 

Meanwhile, $\mD$ is assigned as  $\mD \gets \argmax_{\mI_i} \vpi_{\mI_i}$ during the inference, instead of being sampled from $\vpi$. 
% Thus, it would be sufficient to close the gap by only applying $\appnabla_{\mbox{\scriptsize \oursst}}$ when $\mD$ equals to $\argmax_{\mI_i} \vpi_{\mI_i}$. 
Thus, it would be sufficient to close the gap by only applying $\appnabla_{\mbox{\scriptsize \oursrd}}$ when $\mD \neq \argmax_{\mI_i} \vpi_{\mI_i}$. 
Accordingly, we propose \ours to balance router training and expert training:
\begin{eqnarray*}
\appnabla_{\mbox{\scriptsize \ours}} := (1 - \delta_{\mD}) \appnabla_{\mbox{\scriptsize \oursrd}} + \delta_{\mD} \appnabla_{\mbox{\scriptsize \oursst}}, \mbox{where }  
\delta_{\mD} = 
\begin{cases}
    1,  & \text{if } \mD = \underset{\mI_i}{\argmax}\, \vpi_{\mI_i} \\
    0,  & \text{otherwise} 
\end{cases}.
\end{eqnarray*}

\smallsection{Computational Efficiency of \ours}
$\appnabla_{\mbox{\scriptsize \ours}}$ does not require Hessian or other second-order derivatives, thus having negligible computation overheads (empirical verifications are discussed in Section~\ref{subsec:efficiency}).
At the same time, similar to $\appnabla_{\mbox{\scriptsize ST}}$, our proposed algorithm can be easily integrated with popular library
% automatic differentiation toolkits 
like PyTorch, making it easy to be integrated with existing algorithms. 


==> input/pseudo.tex <==
\begin{minipage}[t*]{0.45\textwidth}
\input{input/pseudo_st}
\end{minipage}
\hfill
\begin{minipage}[t*]{0.52\textwidth}
\input{input/pseudo_sparsemax}
\end{minipage}

==> input/pseudo_sparsemax.tex <==

\begin{algorithm}[h]
\DontPrintSemicolon
\KwIn{$\vtheta$: softmax input,  $\tau$: temperature.}
\KwOut{$\mD$: one-hot samples.}
$\vpi_0 \gets \mbox{softmax}(\vtheta)$ \;
$\mD \gets \mbox{sample\_one\_hot}(\vpi_0)$ \;
$\vpi_1 \gets \frac{\mD + \mbox{softmax}_{\tau}(\vtheta)}{2}$\;
$\vpi_1 \gets \mbox{softmax}\LARGE(\normalsize \mbox{stop\_gradient}(\ln(\vpi_1) - \vtheta) + \vtheta\LARGE)\normalsize$\;
$\vpi_2 \gets 2 \cdot \vpi_1 - \frac{1}{2} \cdot \vpi_0$\;
$\mD \gets \vpi_2 - \mbox{stop\_gradient}(\vpi_2) + \mD$\;
\Return{$\mD$}
\caption{ReinMax. }
\label{algo:reinmax}
\end{algorithm}


==> input/pseudo_st.tex <==

\begin{algorithm}[h]
\DontPrintSemicolon
\KwIn{$\vtheta$: softmax input, $\tau$: temperature, $\{f_i\}$}
\KwOut{$\mD$: one-hot samples.}
$\vpi_0 \gets \mbox{softmax}(\vtheta)$ \;
$\mD \gets \mbox{sample\_one\_hot}(\vpi_0)$ \;
$\vpi_1 \gets \mbox{softmax}_\tau(\vtheta)$\;
\tcc{$\mbox{stop\_gradient}(\cdot)$ duplicates its input and detaches it from backpropagation. }
$\mD \gets \vpi_1 - \mbox{stop\_gradient}(\vpi_1) + \mD$ \;
\Return{$\mD$}
\caption{ST. }
\label{algo:st}
\end{algorithm}

